Neurosymbolic Conformal Classification

The last decades have seen a drastic improvement of Machine Learning (ML), mainly driven by Deep Learning (DL). However, despite the resounding successes of ML in many domains, the impossibility to provide guarantees of conformity and the fragility of ML systems (faced with distribution shifts, adversarial attacks, etc.) have prevented the design of trustworthy AI systems. Several research paths have been investigated to mitigate this fragility and provide some guarantees regarding the behavior of ML systems, among which are neurosymbolic AI and conformal prediction. Neurosymbolic artificial intelligence is a growing field of research aiming to combine neural network learning capabilities with the reasoning abilities of symbolic systems. One of the objective of this hybridization can be to provide theoritical guarantees that the output of the system will comply with some prior knowledge. Conformal prediction is a set of techniques that enable to take into account the uncertainty of ML systems by transforming the unique prediction into a set of predictions, called a confidence set. Interestingly, this comes with statistical guarantees regarding the presence of the true label inside the confidence set. Both approaches are distribution-free and model-agnostic. In this paper, we see how these two approaches can complement one another. We introduce several neurosymbolic conformal prediction techniques and explore their different characteristics (size of confidence sets, computational complexity, etc.).

==> circuits.tex <==
A circuit over variables $\mathbf{Y}$ is a node labeled directed acyclic graph $C=(N, W, \lambda)$ such that:
\begin{itemize}
    \item $N$ is a set of nodes called \textbf{gates}
    \item $W \in N^2$ is a set of edges called \textbf{wires}
    \item $(N, W)$ is directed acyclic graph with a unique sink $g_0 \in N$
    \item $\lambda: N \mapsto \{\land, \lor, \neg, \top, \bot\} \cup \mathbf{Y}$
    \item if $(h, g) \in W$, then gate $h$ is called an \textbf{input} of gate $g$
    \item for all $g \in N$:
    \begin{itemize}
        \item if $\lambda(g) \in \{\top, \bot\}$, then $g$ is a \textbf{constant gate} and has no input
        \item if $\lambda(g) \in \mathbf{Y}$, then $g$ is a \textbf{variable gate} and has no input
        \item if $\lambda(g) = \neg$, then $g$ is a \textbf{negation gate} and has one input
        \item if $\lambda(g) = \land$ (respectively $\lambda(g) = \lor$), then $g$ is a $\land$-gate (respectively $\lor$-gate) must have at least one input
    \end{itemize}
\end{itemize}
The size of a circuit is its number of wires, ie. $|C|:=|W|$.

==> complexitytab.tex <==
% \begin{table}[h]
%     \begin{center}
%     \begin{tabular}{||l|c c c c c||}
%         \hline\hline
%         Classes & Treewidth & Enumerability & SAT & MPE & PQE \\
%         \hline
%         General & $\mathcal{O}(k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ \\
%         \hline
%         2-Horn & $\mathcal{O}(k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ \\
%         \multicolumn{1}{||r|}{Taxonomic} & 1 & $\mathcal{O}(2^k)$ & $\mathcal{O}(1)$ & $\mathcal{O}(k)$ & $\mathcal{O}(k)$ \\
%         \multicolumn{1}{||r|}{Saturated and tree-like HEX} & $\mathcal{O}(k)$ & $\mathcal{O}(k)$ & $\mathcal{O}(1)$ & $\mathcal{O}(k)$ & $\mathcal{O}(k)$ \\
%         Multi-categorical & $\mathcal{O}(k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(1)$ & $\mathcal{O}(k)$ & $\mathcal{O}(k)$ \\
%         Recursive functions & $\tau$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(1)$ & $\mathcal{O}(k2^{\tau})$ & $\mathcal{O}(k2^{\tau})$ \\
%         Exactly l-in-k functions & $\mathcal{O}(k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(1)$ & $\mathcal{O}(k^2)$ & $\mathcal{O}(k^2)$ \\
%         Simple paths in directed graphs & - & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(2^k)$ \\
%         \multicolumn{1}{||r|}{Simple paths in DAG} & $\mathcal{O}(k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(1)$ & $\mathcal{O}(k^3)$ & $\mathcal{O}(k^3)$ \\
%         Matchings & $\mathcal{O}(k)$ & $\mathcal{O}(2^k)$ & $\mathcal{O}(k^d)$ & $\mathcal{O}(k^d)$ & $\mathcal{O}(2^k)$ \\
%         \hline\hline
%     \end{tabular}
%     \caption{Summary of tractability for common classes (under P $\ne$ NP assumption)}
%     \label{tab:summary}
%     \end{center}
% \end{table}

% \begin{table}[h]
%     \begin{center}
%     \begin{tabular}{||l|c c c c c||}
%         \hline\hline
%         Classes & Bounded treewidth & Enumerability & SAT & MPE & PQE \\
%         \hline
%         General & \xmark & \xmark & \xmark & \xmark & \xmark \\
%         \hline
%         2-Horn & \xmark & \xmark & \xmark & \xmark & \xmark \\
%         \multicolumn{1}{||r|}{Taxonomic} & \cmark & \xmark & \cmark & \cmark & \cmark \\
%         \multicolumn{1}{||r|}{Saturated and tree-like HEX} & \xmark & \cmark & \cmark & \cmark & \cmark \\
%         Multi-categorical & \xmark & \xmark & \cmark & \cmark & \cmark \\
%         % Recursive functions & \cmark & \xmark & \cmark & \cmark & \cmark \\
%         Exactly l-in-k functions & \xmark & \xmark & \cmark & \cmark & \cmark \\
%         Simple paths in directed graphs & - & \xmark & \xmark & \xmark & \xmark \\
%         \multicolumn{1}{||r|}{Simple paths in DAG} & \xmark & \xmark & \cmark & \cmark & \cmark \\
%         Matchings & \xmark & \xmark & \cmark & \cmark & \xmark \\
%         \hline\hline
%     \end{tabular}
%     \caption{Summary of tractability for common classes (under P $\ne$ NP assumption)}
%     \label{tab:summary}
%     \end{center}
% \end{table}

\begin{table}[h]
    \centering
    \begin{tabular}{||l| c c c ||}
        \hline\hline
        Logics & Bounded treewidth & MPE & PQE \\
        \hline
        General & \xmark & \xmark & \xmark \\
        \hline
        % 2-Horn & \xmark & \xmark & \xmark & \xmark & \xmark \\
        Tree-like hiearchical & \cmark & \cmark & \cmark \\
        Hierarchical with mutual exclusion & \xmark & \cmark & \cmark \\
        % Multi-categorical & \xmark & \xmark & \cmark & \cmark & \cmark \\
        % Recursive functions & \cmark & \xmark & \cmark & \cmark & \cmark \\
        Fixed cardinal & \xmark & \cmark & \cmark \\
        Simple path in directed graphs & \xmark & \xmark & \xmark \\
        Acyclic simple path & \xmark & \cmark & \cmark \\
        Matchings & \xmark & \cmark & \xmark \\
        \hline\hline
    \end{tabular}
    \caption{Summary of tractability results}
    \label{tab:summary}
\end{table}

==> link.tex <==
\textbf{Fixed cardinal} constraints can be used to represent a classification task which consists in picking a fixed amount of variables in a given list (\eg suggesting a given number of related products to a client).

A fixed cardinal theory consists of a linear constraint $\langle \mathbf{Y}_{1:k}, \mathbf{1} \rangle=l$ which accepts states that contain exactly $l$ variables amongst a set of size $k$ (ie. states $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{1:k}}$ such that $|\mathbf{y}|=l$).

Figures \ref{fig:link_nodes} gives a recursive template (using the graphical representation in \cite{Darwiche2011}) to compile in polynomial time (create all decision nodes and connect them appropriately) a fixed cardinal theory $\langle \mathbf{Y}_{1:k}, \mathbf{1} \rangle=l$ into a \textbf{concise} SDD.

\begin{figure}[htb]
\begin{subfigure}[t]{0.22\linewidth}
    % \centering
    \includegraphics[width=\textwidth]{circuits/link/Node_1in1.png}
    \caption{$C_1^1$}
    \label{fig:link_C11}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.22\linewidth}
    % \centering
    \includegraphics[width=\textwidth]{circuits/link/Node_0in1.png}
    \caption{$C_0^1$}
    \label{fig:link_C01}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.22\linewidth}
    % \centering
    \includegraphics[width=\textwidth]{circuits/link/Node_0ink.png}
    \caption{$C_0^k$}
    \label{fig:link_C0k}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.22\linewidth}
    % \centering
    \includegraphics[width=\textwidth]{circuits/link/Node_link.png}
    \caption{$C_l^k$ for $l>0$}
    \label{fig:link_Clk}
\end{subfigure}
\caption{Decision nodes $C_l^k$}
\label{fig:link_nodes}
\end{figure}

\begin{proposition}
    Circuit $C_l^k$ has size polynomial in $k$.
\end{proposition}

\begin{proof}
    Circuit $C_l^k$ contains nodes $(C_i^j)_{1 \leq j \leq k, 0 \leq i \leq j}$ with $6$ wires each, meaning that the size of the circuit is in $\mathcal{O}(k^2)$.
\end{proof}

\begin{proposition}
    For any number of variables $k \geq 1$ and $0 \leq l \leq k$ the circuit rooted in $C_l^k$ is a SDD (and even an OBDD) structured according to the right linear vtree on $\mathbf{Y}_{1:k}$.
\end{proposition}

\begin{proof}
    Proof by recurrence on $k$ starting at $k=1$:
    \begin{itemize}
        \item Initialization for $k=1$: $C_1^1$ and $C_0^1$ only contains variable $Y_1$ and thus is structured according to the right linear vtree on $Y_1$.
        \item Heredity from $k$ to $k+1$: for all $0 \leq l \in k+1$, $C_l^{k+1}$ has primes $\{Y_{k+1}, \neg Y_{k+1}\}$ and subs $\{C_{l-1}^k, C_l^k\}$ if $l>0$ and $\{C_0^k, \bot\}$ if $l=0$ which are all structured according to the right linear vtree on $\mathbf{Y}_{1:k}$, hence $C_l^{k+1}$ is structured according to the right linear vtree on $\mathbf{Y}_{i:k+1}$.
    \end{itemize}
\end{proof}

\begin{proposition}
    The circuit $C_l^k$ with $k \geq 1$ and $0 \leq l \leq k$ accepts a state $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{i:k}}$ iff it contains exactly $l$ variables (ie. $|\mathbf{y}|=l$).
\end{proposition}

\begin{proof}
    Proof by recurrence on $k$ starting at $k=1$:
    \begin{itemize}
        \item Initialization for $k=1$: $C_1^1$ only accepts $y_1=1$ and $C_0^1$ only accepts $y_1=0$.
        \item Heredity from $k$ to $k+1$, for $0 \leq l \leq k$ and $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{i:k+1}}$:
        \begin{itemize}
            \item if $l=0$: $C_0^{k+1}(\mathbf{y})=1$ iff $y_{k+1}=0$ and $C_0^k(\mathbf{y}_{i:k})=1$, which means $C_0^{k+1}$ accepts $\mathbf{y}$ iff:
            $$|\mathbf{y}|=|\mathbf{y}_{i:k}|+y_{k+1}=0+0=0$$
            \item if $l>0$: $C_l^{k+1}(\mathbf{y})=1$ in only two cases:
            \begin{itemize}
                \item if $y_{k+1}=0$ and $C_l^k(\mathbf{y}_{i:k})=1$, which means we have: $$|\mathbf{y}|=|\mathbf{y}_{i:k}|+y_{k+1}=l+0=l$$
                \item if $y_{k+1}=1$ and $C_{l-1}^k(\mathbf{y}_{i:k})=1$, which means we have: $$|\mathbf{y}|=|\mathbf{y}_{i:k}|+y_{k+1}=l-1+1=l$$
            \end{itemize}
        \end{itemize}
    \end{itemize}
\end{proof}

==> paths.tex <==
The task of Warcraft Shortest Path \cite{pogancic_differentiation_2019} is to learn how to predict the shortest path on a map from a picture of the map. Such a task can be viewed as an informed classification task where the set of output variables correspond to edges in a graph and prior knowledge informs us that only states representing simple paths in the graph are satisfying answers.

\textbf{Simple path} logic $\mathcal{L}_{\bullet \to \bullet}:=(\mathcal{T}_{\to}, \mathscr{s}_{\bullet \to \bullet})$ is an edge-based logic where a theory $(G:=(V, E), \varsigma)$ accepts a state $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}}$ if the edges selected in $E$ (ie. $\{e \in E | \varsigma(e) \in \mathbf{y}\}$) form a s-t simple path in $G$, \ie if the selected edges forms an acyclic path from a source of the graph to a target (or sink) of the graph.
\vspace{5mm}
% A \textbf{simple path} boolean functions accepts states that correspond to a simple path (sometimes called a self-avoiding path) in a directed graph. Assume a directed graph $D=(V, E)$ with $|E|=k$ edges, an ordering of the edges $\sigma$, a source node $s \in V$ and a target node $t \in V$. We note $e_j$ the edge such that $\sigma(e)=j$. The boolean function $\mathscr{f}_{D[s \to t]}$ accepts states $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{1:k}}$ for which the collection of edges in $\mathbf{y}$ (ie. $(e_j)_{Y_j \in \mathbf{y}}$) forms a simple path in $D$.

% Simple path boolean functions can be expressed in ASP logic with programs composed of the rules:
% \begin{gather}
%     r_{(s, u)} : Y_{(s, u)} \leftarrow (\text{\textit{not} } Y_{(s, v)})_{\substack{(s, v) \in E \\ v \ne u}} \text{ \textit{for} } (s, u) \in E \\
%     r_{(v, w)} : Y_{(v, w)} \leftarrow (Y_{(u, v)})_{(u, v) \in E}  \text{ \textit{for} } v \in V \setminus s, (v, w) \in E
% \end{gather}

\begin{proposition}
    Simple path logic is MPE and PQE-intractable.
\end{proposition}

\begin{proof}
    Solving MPE for a simple path theory $(G, \varsigma)$ is equivalent to finding a shortest path in $G$ with real weights on the edges, which is known to be NP-hard by a polynomial reduction from the Hamiltonian path problem \cite{Karp1972}. Likewise, counting the number of simple paths of a graph $G$ is known to be \#P-hard \cite{valiant1979} and has a trivial polynomial reduction to solving PQE for a simple path theory $(G, \varsigma)$.
\end{proof}

A simple path theory $(D, \varsigma)$ is said \textbf{acyclic} if $D$ is a Directed Acyclic Graph (DAG). We say that $(D, \varsigma)$ is \textbf{topological} if $\varsigma$ is a topological ordering of the edges: for any path, the order of edges in the path is a sub-order of the topological order. For a vertex $u \in V$, we will note $\varsigma_m(u)$ the index of the first incident edge to $u$ and $\varsigma_M(u)$ the index of the last outgoing edge of $u$. We also note $D^j$ the graph that contains edges $(e_i)_{1 \leq i \leq j}$ and all vertices that are endpoints of those edges. Finally, we can assume without loss of generality that $D$ only contains a single source and target. If not: chose one source vertex $s$, delete all the others and reconnect their outgoing edges to $s$, and do the same with a target vertex $t$. This operation can be done in polynomial type and does not change the semantic of the theory (\ie accepted states are left unchanged).

Figures \ref{fig:spk_nodes} and \ref{fig:spi_nodes} represent recursive templates that allow us to compile in polynomial time (create all decision nodes and connect them appropriately) an acyclic and topological simple path theory $(D:=(V, E), \varsigma)$ into a \textbf{concise} SDD rooted in node $C_t^k$.
\vspace{5mm}
\begin{figure}[b]
\begin{subfigure}[t]{0.30\linewidth}
    \centering
    \includegraphics[width=\textwidth]{circuits/paths/FinalIncomingNode.png}
    \caption{{\scriptsize $C_v^1$ if $e_1=(s, v)$}}
    \label{fig:Cnk_outgoing}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.30\linewidth}
    \centering
    \includegraphics[width=\textwidth]{circuits/paths/FinalNode.png}
    \caption{{\scriptsize $C_v^1$ if $v \neq s$ and $e_1 \neq (s, v)$}}
    \label{fig:Cnk}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.30\linewidth}
    \centering
    \includegraphics[width=\textwidth]{circuits/paths/FinalSourceNode.png}
    \caption{{\scriptsize $C_s^1$}}
    \label{fig:Cs1}
\end{subfigure}
\caption{Initial decision nodes $C_v^1$ for $v \in V$}
\label{fig:spk_nodes}
\end{figure}

\begin{figure}[t]
\hspace*{\fill}
\begin{subfigure}[t]{0.30\linewidth}
    \centering
    \includegraphics[width=\textwidth]{circuits/paths/IncomingNode.png}
    \caption{{\scriptsize $C_v^{i+1}$ if $e_{i+1}=(u, v)$}}
    \label{fig:Cni_outcoming}
\end{subfigure}
\hfill
\begin{subfigure}[t]{0.30\linewidth}
    \centering
    \includegraphics[width=\textwidth]{circuits/paths/NotIncomingNode.png}
    \caption{{\scriptsize $C_v^{i+1}$ if $e_{i+1}$ is not an incoming edge of $v$}}
    \label{fig:Cni_not_outcoming}
\end{subfigure}
\hspace*{\fill}
\caption{Decision nodes $C_v^i$ for $1 < i \leq k$ and $v \in V$}
\label{fig:spi_nodes}
\end{figure}

\begin{proposition}
    Circuit $C_t^k$ has size polynomial in the number of edges in $k$.
\end{proposition}

\begin{proof}
    Circuit $C_t^k$ has at most $|V| \times k = \mathcal{O}(k^3)$ decision nodes with $6$ wires each, meaning that the size of the circuit is in $\mathcal{O}(k^3)$.
\end{proof}

\begin{remark}
    Notice that every node $C_v^i$ such that such that $i > \sigma_M(v)$ will not appear in the circuit rooted in $C_t^k$. Similarly, every node $C_v^i$ such that $i < \sigma_m(v)$ is equivalent to $\bot$ and can thus be trimmed of the circuit. Therefore, the size of the trimmed circuit is much smaller that $2k^3$.
\end{remark}

\begin{proposition}
    For each vertex $v$ and edge $e_i$, the circuit rooted in $C_v^i$ is a SDD (and even an OBDD) structured according to the right linear vtree on $\mathbf{Y}_{1:i}$.
\end{proposition}

\begin{proof}
    Proof by recurrence on $i$:
    \begin{itemize}
        \item Initialization for $i=1$: for all vertices $v$, $C_v^1$ only contains variable $Y_1$ and thus is structured according to the right linear vtree on $Y_1$.
        \item Heredity from $i$ to $i+1$: for all vertices $u$, $C_v^i$ has primes $\{Y_i, \neg Y_i\}$ and subs $\{C_u^{i-1}, C_v^{i-1}, \bot\}_{u \in V, (u, v) \in E}$ which are all structured according to the right linear vtree on $\mathbf{Y}_{1:i+1}$, hence $C_v^i$ is structured according to the right linear vtree on $\mathbf{Y}_{1:i}$.
    \end{itemize}
\end{proof}

\begin{lemma} \label{lem:topo}
    Assume that edges follow a topological order. If for $i>1$ $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{1:i}}$ represents a path $s \to v$ in $D^i$ and $y_i=1$, then $e_i=(u, v)$ for some $u \in D^{i-1}$.
\end{lemma}

\begin{proof}
    We note $e_i=(u, w)$. We first show that $u \in D^{i-1}$:
    \begin{itemize}
        \item if $u=s$, then $u \in D^1 \subset D^{i-1}$.
        \item if $u \ne s$, since $\mathbf{y}$ represents a path $s \to v$, there is an edge $e_j=(r, u)$ with $j < i$, which means that $u \in D^{i-1}$. 
    \end{itemize}
    
    Now let's show that $w=v$ reasoning by the absurd. Let's assume that $w \ne v$, then since $\mathbf{y}$ represents a path $s \to v$, there is an edge $e_l=(q, v)$ with $l<i$. Hence, there is a path from the end point $w$ of $e_i$ to the start point $q$ of $e_l$ with $l<i$, which is in contradiction with edges following a topological order.

    Therefore we can conclude that $e_i=(u, v)$ for some $u \in D^{i-1}$.
\end{proof}

\begin{lemma} \label{lem:Csi}
    The circuit $C_s^i$ with $1 \leq i \leq k$ only accepts the null state $\mathbf{0} \in \mathbb{B}^{\mathbf{Y}_{1:i}}$.
\end{lemma}

\begin{proof}
    Proof by recurrence on $i$:
    \begin{itemize}
        \item Initialization for $i=1$: $C_s^{1}(y_1)=1$ iff $y_1=0$ by definition (see Figure \ref{fig:Cs1}).
        \item Heredity from $i$ to $i+1$: $s$ has no incoming edge in $D$ (because it is a source vertex), hence $C_s^{i+1}$ accepts $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{1:i+1}}$ iff $y_{i+1}=0$ and $C_s^{i}(\mathbf{y}_{1:i})=1$. Which means by the recurrence hypothesis that $\mathbf{y}_{1:i}=\mathbf{0}$ and therefore $\mathbf{y}=0$.
    \end{itemize}
\end{proof}

\begin{proposition}
    The circuit $C_v^i$ with $1 \leq i \leq k$ and $v \in D^i \setminus s$ accepts a state $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{1:i}}$ iff it is a path $s \to v$ in $D^i$. In particular $C_t^k$ represents $\mathscr{f}_{D[s \to t]}$.
\end{proposition}

\begin{proof}
    We will proceed by recurrence on $i$, first showing that all accepted states by $C_v^i$ are paths $s \to v$ in $D^i$ then showing that only them are accepted.
    \begin{itemize}
        \item Initialization for $i=1$: $D^1$ only contains the vertices $s$ and $v$ such that $e_1=(s, v)$ and $C_v^1$ accepts exactly $y_1=1$ which is the only path $s \to v$ in $D^1$.
        \item Heredity from $i$ to $i+1$:
        \begin{itemize}
            \item Assume a state $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{1:i+1}}$ represents a path $s \to v$ in $D^{i+1}$ and note:
            \begin{itemize}
                \item if $y_{i+1}=1$, then according to Lemma \ref{lem:topo} $e_{i+1}=(u, v)$ for some $u \in D^i$
                \begin{itemize}
                    \item if $u=s$: then $\mathbf{y}_{1:i}=\mathbf{0}$ and by Lemma \ref{lem:Csi} $C_v^{i+1}(\mathbf{y})=C_s^{i}(\mathbf{y}_{1:i})=1$
                    \item if $u \ne s$: then $\mathbf{y}_{1:i}$ represents a path $s \to u$ in $D^i$ and by the recurrence hypothesis $C_v^{i+1}(\mathbf{y})=C_u^i(\mathbf{y}_{1:i})=1$
                \end{itemize}
                \item if $y_{i+1}=0$, then $\mathbf{y}_{1:i}$ represents a path $s \to v$ in $D^i$ and by the recurrence hypothesis $C_v^{i+1}(\mathbf{y})=C_v^i(\mathbf{y}_{1:i})=1$.
            \end{itemize}
            \item Assume a state $\mathbf{y} \in \mathbb{B}^{\mathbf{Y}_{1:i+1}}$ is accepted by $C_v^{i+1}$:
            \begin{itemize}
                \item if $y_{i+1}=1$, then according to Lemma \ref{lem:topo} $e_{i+1}=(u, v)$ for some $u \in D^i$
                \begin{itemize}
                    \item if $u=s$: then $C_s^{i}(\mathbf{y}_{1:i})=C_v^{i+1}(\mathbf{y})=1$, hence by Lemma \ref{lem:Csi} $\mathbf{y}_{1:i}=\mathbf{0}$ and $\mathbf{y}$ represents a path $s \to v$ in $D^{i+1}$.
                    \item if $u \ne s$: then $C_u^i(\mathbf{y}_{1:i})=C_v^{i+1}(\mathbf{y})=1$, hence by the recurrence hypothesis $\mathbf{y}_{1:i}$ represents a path $s \to u$ in $D^i$ and by adding $e_{i+1}$ $\mathbf{y}$ represents a path $s \to v$ in $D^{i+1}$.
                \end{itemize}
                \item if $y_{i+1}=0$, then $C_u^i(\mathbf{y}_{1:i})=C_u^{i+1}(\mathbf{y})=1$, hence by the recurrence hypothesis $\mathbf{y}_{1:i}$ represents a path $s \to v$ in $D^i$ and by not adding edge $e_{i+1}$ $\mathbf{y}$ represents a path $s \to v$ in $D^{i+1}$.
            \end{itemize}
        \end{itemize}
    \end{itemize}
\end{proof}

Finally, we can state our main result:
\vspace{5mm}
\begin{proposition}
    The fragment of simple path logic composed of acyclic theories is tractable.
\end{proposition}

\begin{proof}
    First, it is concise because it is an edge-based logic. Let's assume an acyclic simple path theory $(G, \varsigma)$. If needed, merge source vertices and target vertices like mentioned above. Since a topological order of the edges in a DAG can be compiled in a polynomial time, we can compute $\varrho$ such that $(G, \varrho)$ is acyclic and topological. We compile $(G, \varrho)$ into a concise SDD $C_t^k$ as seen above. We rewrite leaf nodes $Y_i$ to $Y_{\varsigma \circ \varrho^{-1}(i)}$ in the SDD. The new circuit is still a concise SDD, structured according to the right linear vtree on $(Y_{\varsigma \circ \varrho^{-1}(i)})_{1 \leq i \leq k}$ and is equivalent to the theory $(G, \varsigma)$. Because SDD is MPE and PQE-tractable, we have that acyclic simple path logic is concise, MPE and PQE-tractable. Therefore, acyclic simple path logic is tractable.
\end{proof}


% Let's first give to quick lemmas about circuit $C_s^1$:
% \begin{enumerate}
%     \item a node $C_{v_p}^i$ does not accept a state $\mathbf{y} \in \mathbb{B}^{\mathbf{E}}$ if there is $j>i$ such that all nodes $C_{v_q}^j$ where $v_q$ does not precede $v_p$ in the order (ie. $q \geq p$) does not accept $\mathbf{y}$:
%     \begin{equation}
%         \forall 1\leq i < k, 1 \leq p < m, (\exists j>i, \forall q \geq p, C_{v_q}^j(\mathbf{y}_{j:k})=0) \implies C_{v_p}^i(\mathbf{y}_{i:k})=0
%     \end{equation}
%     \item a node $C_{v_p}^i$ does not accept a state $\mathbf{y} \in \mathbb{B}^{\mathbf{E}}$ if there is a later vertice $v_q$ (ie. $q>p$) such that for all edges $e_j$ the node $C_{v_q}^j$ does not accept $\mathbf{y}$:
%     \begin{equation}
%         \forall 1\leq i < k, 1 \leq p < m, (\exists q>p, \forall 1\leq j  k, C_{v_q}^j(\mathbf{y}_{j:k})=0) \implies C_{v_p}^i(\mathbf{y}_{i:k})=0
%     \end{equation}
% \end{enumerate}

% \begin{lemma} \label{lem:non_terminal}
%     A non-terminal node $C_{v_p}^i$ (ie. where $i<k$) can only accept a state if one of the following nodes $(C_{v_q}^{i+1})_{p \leq q \leq m}$ accepts it.
% \end{lemma}

% \begin{lemma} \label{lem:disconnect}
%     If there is a edge $e_j$ and a vertice $v_p$ such that for all vertices $v_q$ after $v_p$ (ie. $p \leq q$) the node $C_{v_q}^j$ rejects a state $\mathbf{y}$, then for any previous edge $e_i$ (ie. $i \leq j$) and for all vertices $v_q$ after $v_p$ the node $C_{v_q}^i$ also rejects $\mathbf{y}$:
%     \begin{gather} \label{eq:disconnect}
%         \forall 1 \leq j \leq k, 1 \leq p \leq m, \forall \mathbf{y} \in \mathbb{B}^{\mathbf{E}} \notag \\
%         (\forall p \leq q \leq m, C_{v_q}^j(\mathbf{y}_{j:k})=0) \implies (\forall 1 \leq i \leq j, \forall p \leq q \leq m, C_{v_q}^i(\mathbf{y}_{i:k})=0)
%     \end{gather}
% \end{lemma}

% \begin{proof}
%     Assume $1 < j \leq k, 1 \leq p \leq m$ and $\mathbf{y} \in \mathbb{B}^{\mathbf{E}}$ such that:
%     \begin{equation*}
%         \forall p \leq q \leq m, C_{v_q}^j(\mathbf{y}_{j:k})=0
%     \end{equation*}
    
% Let's show by recurrence on $i$ starting at $i=j$ and ending at $i=1$, that:
%     \begin{equation}
%         \forall 1 \leq i \leq j, \forall p \leq q \leq m, C_{v_q}^i(\mathbf{y}_{i:k})=0
%     \end{equation}
%     \begin{itemize}
%         \item Initialization at $i=j$: direct from the hypothesis.
%         \item Heredity from $i+1 \leq j$ to $i$: all nodes in $(C_{v_q}^{i+1})_{p \leq q \leq m}$ reject $\mathbf{y}$, hence applying Lemma \ref{lem:non_terminal} on any node in $(C_{v_q}^{i})_{p \leq q \leq m}$ gives you: $\forall p \leq q \leq m, C_{v_q}^i(\mathbf{y}_{i:k})=0$.
%     \end{itemize}
% \end{proof}

% \begin{lemma} \label{lem:2out}
%     If there is is a vertice $v_d$ with two outcoming edges $e_i$ and $e_j$ ($i<j$) in a state $\mathbf{y}$, then $C_s^1(\mathbf{y})$ rejects $\mathbf{y}$.
% \end{lemma}

% \begin{proof}
%     Assume that there is a vertice $v_d$ with two outcoming edges $e_i=(v_d, v_p)$ and $e_j$ ($i<j$) in $\mathbf{y}$. Let's first show that $C_{v_p}^{i+1}(\mathbf{y}_{i+1:k})=0$:
%     \begin{itemize}
%         \item If $j=i+1$, then because $y_j=1$ and $e_j$ is not an outcoming edge of $v_p$: $C_{v_p}^{i+1}(\mathbf{y}_{i+1:k})=0$.
%         \item If $j > i+1$, then for all $p \leq q \leq m$: $e_j$ is not an outcoming edge of $v_q$, which implies $C_{v_q}^j(\mathbf{y}_{j:k})=0$ since $y_j=1$. Following Lemma \ref{lem:disconnect}, this leads to: $$\forall 1 \leq l \leq j, \forall p \leq q \leq m, C_{v_q}^l(\mathbf{y}_{l:k})=0$$ and in particular to $C_{v_p}^{i+1}(\mathbf{y}_{i+1:k})=0$.
%         % \begin{equation*}
%         %     \forall 1 \leq i \leq j, \forall p \leq q \leq m, C_{v_q}^i(\mathbf{y}_{i:k})=0
%         % \end{equation*}
%     \end{itemize}

%     Since $y_i=1$, $e_i=(v_d, v_p)$ and $C_{v_p}^{i+1}(\mathbf{y}_{i+1:k})=0$, we have: $C_{v_d}^i(\mathbf{y}_{i:k})=0$. Besides, because $y_i=1$ and $e_i$ is not an outcoming edge for all other vertices than $v_d$, then: $$\forall 1 \leq q \ne d \leq m, C_{v_q}^i(\mathbf{y}_{i:k})=0$$

%     Combining both gives:
%     \begin{equation*}
%         \forall 1 \leq q \leq m, C_{v_q}^i(\mathbf{y}_{i:k})=0
%     \end{equation*}

%     Applying Lemma \ref{lem:disconnect} we get:
%     \begin{equation*}
%         \forall 1 \leq l \leq i, \forall 1 \leq q \leq m, C_{v_q}^l(\mathbf{y}_{l:k})=0
%     \end{equation*}

%     In particular with $l=q=1$ this gives: $C_s^1(\mathbf{y})=C_{v_1}^1(\mathbf{y})=0$.
% \end{proof}

% \begin{lemma} \label{lem:1in1out}
%     If there is a non-target vertice $v_d$ (ie. $d<m$) with an incoming edges $e_i$ and no outcoming edges in a state $\mathbf{y}$, then $C_s^1(\mathbf{y})$ rejects $\mathbf{y}$.
% \end{lemma}

% \begin{proof}
%     Assume that $v_d$ is the first vertice with an incoming edges $e_i$ and no outcoming edges in a state $\mathbf{y}$.
    
%     Let's first show by recurrence on $j$ from $j=k$ to $j=i$ that: $$\forall i \leq j \leq k, C_{v_d}^i(\mathbf{y}_{i:k})=0$$
%     \begin{itemize}
%         \item Initialization $j=k$:
%         \begin{itemize}
%             \item if $e_k=(v_d, t)$, then $y_k=0$ from the hypothesis and $C_{v_d}^k(y_k)=0$
%             \item if $e_k \ne (v_d, t)$, then $C_{v_d}^k(y_k)=0$ by default
%         \end{itemize}
%         \item Heredity from $j+1$ to $j$:
%         \begin{itemize}
%             \item if $e_j=(v_d, v_p)$, then $y_j=0$ from the hypothesis and: $$C_{v_d}^j(\mathbf{y}_{j:k})=C_{v_d}^{j+1}(\mathbf{y}_{j+1:k})=0$$
%             \item if $e_j$ in not an outcoming edge of $v_d$:
%             \begin{itemize}
%                 \item if $y_j=0$: $C_{v_d}^j(\mathbf{y}_{j:k})=C_{v_d}^{j+1}(\mathbf{y}_{j+1:k})=0$
%                 \item if $y_j=1$: $C_{v_d}^j(\mathbf{y}_{j:k})=0$ by default
%             \end{itemize}
%         \end{itemize}
%     \end{itemize}

% \end{proof}


% \begin{enumerate}
%     \item assume there is no outcoming edge of $s$ in $\mathbf{y}$: then by recurrence on nodes $C_s^i$ from $k$ to $1$ $C_s^1(\mathbf{y})=0$.
%     \item assume that there is a node $v_p$ with two outcoming edges $e_i=(v_p, v_q)$ and $e_j$ ($i<j$) in $\mathbf{y}$. Let's  : then $\forall d \geq q, C_{v_d}^j(\mathbf{y}_{j:k})=0$ (because $y_j=1$ and $e_j$ is not an outcoming edge of $v_d$). Follwing Equation \ref{eq:disconnect} this implies that $C_{v_q}^i(\mathbf{y}_{i:k})=0$. Since $y_i=1$, this also implies  and $e_i$ is not an outcoming edge for all other vertices, then $\forall 1 \leq q \leq m$, $C_{v_q}^i(\mathbf{y}_{i:k})=0$, which again from Equation \ref{eq:disconnect} implies $C_s^1(\mathbf{y})=0$.
%     \item assume that there is a node $v_p$ with an incoming edge but no outcoming edge in $\mathbf{y}$:
% \end{enumerate}

% First, assume there is no outcoming edge of $s$ in $\mathbf{y}$: then by recursion on nodes $C_s^i$ from $k$ to $1$ $C_s^1$ evaluates to $\bot$ which is contradictory. Thus there is an outcoming edge of $s$ in $\mathbf{y}$.
% Then assume that there is a node $n$ with two outcoming edges in $\mathbf{y}$.
% Then assume that there is a node $n$ with an incoming edge but no outcoming edge in $\mathbf{y}$.
